Customizing Language Models with Instance-wise LoRA for Sequential Recommendation

Sequential recommendation systems predict the next interaction item based on users' past interactions, aligning recommendations with individual preferences. Leveraging the strengths of Large Language Models (LLMs) in knowledge comprehension and reasoning, recent approaches are eager to apply LLMs to sequential recommendation. A common paradigm is converting user behavior sequences into instruction data, and fine-tuning the LLM with parameter-efficient fine-tuning (PEFT) methods like Low-Rank Adaption (LoRA). However, the uniform application of LoRA across diverse user behaviors is insufficient to capture individual variability, resulting in negative transfer between disparate sequences. To address these challenges, we propose Instance-wise LoRA (iLoRA). We innovatively treat the sequential recommendation task as a form of multi-task learning, integrating LoRA with the Mixture of Experts (MoE) framework. This approach encourages different experts to capture various aspects of user behavior. Additionally, we introduce a sequence representation guided gate function that generates customized expert participation weights for each user sequence, which allows dynamic parameter adjustment for instance-wise recommendations. In sequential recommendation, iLoRA achieves an average relative improvement of 11.4\% over basic LoRA in the hit ratio metric, with less than a 1\% relative increase in trainable parameters. Extensive experiments on three benchmark datasets demonstrate the effectiveness of iLoRA, highlighting its superior performance compared to existing methods in mitigating negative transfer and improving recommendation accuracy. Our data and code are available at https://github.com/AkaliKong/iLoRA.

==> backup/1_introduction.tex <==
\section{Introduction} 
% Sequential recommendation \cite{Session-basedRec, PerSeqRec, SASRec, SeqRecSys, DL4SeqRec} is to predict the next item of interest that aligns the user preferences, based on his/her historical interaction sequences. 
Sequential recommendation \cite{GRU4Rec, PerSeqRec, SASRec, SeqRecSys, DL4SeqRec}  predicts a user's next item of interest by analyzing his/her historical interactions, thereby align closely with individual preferences.
As Large Language Models (LLMs) \cite{LLMsfew-shotLearners, Llama} demonstrate impressive capabilities in global knowledge and reasoning, their potential applications in sequential recommendation are attracting attention \cite{M6-Rec, RLP, TextIsAllYouNeed, TallRec, GenRec, Uncovering, IsGPTGood, LLMzero-shotRanker}. Recent studies \cite{LlaRA, E4SRec} reshape sequential recommendation as language generation tasks, transforming the user behavior sequences into textual input prompts mostly through two distinct trajectories:  fine-tuning LLMs based on pure textual prompts of user behaviors \cite{RLP, TallRec, LlamaRec, InstructionFollowing, GenRec} or hybrid prompts integrated with behavioral tokens \cite{LlaRA, E4SRec, CoLLM, GenRec}.

Regardless of various trajectories, the common paradigm of fine-tuning is a combination of three subsequent components: (1) convert a sequence of historical behaviors into a prompt; (2) collect such prompts with the next items of interest as the instruction-tuning data; (3) apply a Low-Rank Adaptation of Large Language Models (LoRA) module, a widely-used strategy of Parameter-Efficient Fine-Tuning (PEFT), across all the prompts to tune LLMs. Previous studies \cite{P5, RLP, InstructionFollowing, GenRec, LlaRA, E4SRec, CoLLM} primarily focus on optimizing prompts to better incorporate recommendation information, while overlooking the improvements to LoRA. Instead, they rely on a standard LoRA module to fine-tune the model, which freezes the LLM weights and decomposes the updating weights into two additional trainable low-rank matrices.

\wx{However, as user behaviors often exhibit substantial individual variability (\eg distinct interests \cite{xx}, behavior patterns \cite{xx}, feedback mechanisms \cite{xx}), we argue that employing a uniform LoRA module across such diverse behaviors may not capture these variabilities effectively.
Specifically, the variability in user behaviors naturally inspires us to view individual sequential recommendations as different tasks. Simply applying a singular LoRA module leaves this multitask nature of sequential recommendation untouched, thus potentially overestimating the relationships between sequences. It easily causes the negative transfer between significantly discrepant sequences. Take LLaRA as an example, which fine-tunes a LoRA module on top of LLaMA-2 across all sequences. Following prior studies \cite{Gradient vaccine,C-Poly}, we analyzed the gradients of LLaRA associated with disparate sequences, as shown in Figure \ref{fig:motivation}. Clearly, such gradients are misaligned, which can lead to suboptimal performance. To mitigate this issue, one straightforward solution is to implement multiple LoRA modules, with each module fine-tuned for a specific sequence, allowing each module to act as a lightweight expert tailored to its respective sequence.
However, it is impractical in terms of resources and time complexity as the number of sequences typically scales to millions.
}


However, as user behaviors often display substantial individual variability (\eg distinct interests \cite{xx}, behavior patterns \cite{xx}, feedback mechanisms \cite{xx}), we argue that simply employing a uniform LoRA module across different user behaviors may not adequately capture such variabilities.
To address the limitation, exploring more sophisticated LoRA modules instead to customize LLMs for distinct behavioral sequences is a promising research direction. However, Some challenges must be taken into consideration:
% 1st complexity 2nd cost 3rd generalization-capability
\begin{itemize}[leftmargin=*]
% \item \textbf{Problem Complexity.} Recommendation system is tasked with interpreting complex and dynamic user behaviors that exhibit high variability across different user segments. It's difficult for a singular set of parameters to finely capture the intrinsic characteristics. This complexity needs a solution that can segment the overarching problem into more discrete components, each tailored to specific patterns of user behavior.
\item \textbf{Problem Complexity.} To better interpret complex and variable user behaviors, Previous methods often employ clustering techniques to categorize users.
However, this approach tends to learn more towards multi-mode recommendation rather than achieving a fully sequence-tailored recommendation.
To overcome the limitation, it's essential to implements a system that dynamically adapts to each unique behavior sequence, recognizing subtle shifts in preference.
% 2 删掉？提了两次clustering
\item \textbf{Cost Concerns.} Previously, clustering users and training a dedicated sequential model for each group is a circuitous way. Yet, in the era of LLMs, the prohibitive costs of fine-tuning make it economically unfeasible. An efficient strategy would, therefore, need to utilize shared learning architectures that can operate across multiple user demographics, thereby reducing redundancy and maximizing resource utilization.
\item \textbf{Generalization Capabilities.} Ensuring that a model generalizes well is significant. A singular model approach often has trouble balancing between overfitting some data segments and underperforming on others. The ideal strategy would involve integrating insights from various specialized experts, each fine-tuned to distinct facets of the dataset.
\end{itemize}


% Our core idea is dynamically adjusting the parameters of LoRA based on the similarity of user behavior sequences --- shifting from a one-for-all to a one-for-one recommendation paradigm. 

% unlike traditional explicit task segmentation in MOE methods, we innovatively treat the next-item-prediction of all sequences as a form of multitask learning, using historical interaction representations in sequence space as a basis. 
% The main idea of MOE is to decompose complex problems into multiple sub-problems, each addressed by a group of experts. With a gating network assessing the data and determining which experts are most suitable for the current input, it ultimately aggregates these experts’ responses based on weighted contributions to form the final output.

To deal with these challenges, we turn our attention on combining LoRA with the Mixture of Experts 
(MOE) \cite{MOE1, MOE2} method and propose a simple yet effective method called \textbf{S}equence-\textbf{TA}ilored \textbf{Rec}ommendation \textbf{(STARec)}. 
% constructing custom LoRA parameter activation patterns for each sequence through soft routing.
% Specifically, we refine the classic LoRA method by implementing fine-grained segmentation of experts, enhancing the precision of user preference control, while concurrently keeping training costs in check. Additionally, for each matric set $\mathbf{A}$ and $\mathbf{B}$, we incorporate a gating network to determine the weight of each expert’s contribution to the final output. To implicitly decompose sequence data into sub-tasks and enable the collaborative signals of traditional sequential models to guide LLMs at a parameter level for customized sequential recommendation tasks, we input users’ historical interaction sequences into traditional recommendation systems to generate a sequence representation enriched with synergistic information. The embedding is then used as input to direct the gating network, which outputs customized expert participation weights for activating LoRA on an instance-by-instance basis. Therefore, \textbf{STARec} deeply leverages the collaborative information from traditional sequential models to guide LLMs in tailoring recommendations that more closely match user preferences. We assess the effectiveness of \textbf{STARec} through extensive experiments on three benchmark datasets and comparisons with existing methods.
Specifically, Our framework follows the basic scheme of LoRA, finely segmenting each pair of low-rank matrices, thereby yielding a diverse array of experts. Inspired by MOE, each expert has the potential to glean insights into specific user preferences. 
% Moreover, such approach, while maintaining a relatively constant parameter count, unlocks the capability to tailor activation weights for distinct sequences.
Moreover, such approach keeps the overall parameter count relatively constant while providing the potential to tailor activation weights for distinct sequences.
Subsequently, to cater to the diverse traits observed in user sequences and tailor distinct training and inference strategies, we introduce a sequence-representation-motivated gate function. Specifically, we input users’ historical interaction sequences into traditional recommendation systems to generate a sequence representation enriched with synergistic information. The embedding is then used as input to direct the gating network, which outputs customized expert participation weights for activating LoRA on an instance-by-instance basis. Therefore, \textbf{STARec} deeply leverages the collaborative information to guide LLMs in tailoring recommendations that more closely match user preferences. We assess the effectiveness of \textbf{STARec} through extensive experiments on three benchmark datasets and comparisons with existing methods.

==> backup/2_preliminary.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=1\textwidth]{figures/motivation3.png}
%     \caption{This figure presents the gradient similarity of LoRA modules across all training steps. We utilized signals from the collaborative space to partition the sequence dataset into 8 clusters. Euclidean distance was employed to gauge the proximity between clusters, while gradient similarity was measured to assess geometric loss. Clusters that are closer in the collaborative space are depicted as closer together in the figure, with darker-colored cells indicating higher gradient similarity.}
%     \label{fig:motivation}
% \end{figure}


\section{Preliminary}

% \textbf{Task Formulation.}
\textbf{LLM-based Sequential Recommendation}
The primary task of sequential recommendation is to predict the next item that aligns with user preference \cite{DL4SeqRec, SeqRecSys}.
Formally, consider a user with a historical interaction sequence represented as $\Mat{i}_{< n} = [i_1, i_2,...,i_{n-1}]$, where each $i_j$ is an item interacted with at the $j$-th step.
A sequential recommender, parameterized by $\theta$, inputs this sequence and outputs a probability distribution over potential next items in the candidate set. This model is trained to maximize the likelihood of the true next item $i_{n}$:
\begin{equation}
    \max_{\theta} \sum_{\mathcal{D}} \log P_{\theta}(i_{n} | \Mat{i}_{< n}),
\end{equation}
% where $i_{\leq n}$ represents the sequence of interactions prior to timestep $n$.
In the context of LLM-based sequential recommendation, we employ instruction tuning \cite{zero-shotLearners, T5}, which fine-tunes LLMs using training data structured into explicit instructional pairs $(\bm{x}, \bm{y})$. Here, $\Mat{x}$ comprises a detailed textual instruction describing the interaction sequences $\Mat{i}_{< n}$ and recommendation task \cite{P5, TallRec, LlamaRec, LlaRA, CoLLM, E4SRec}, and $\Mat{y}$ is the textual description of the predictive item $i_{n}$ in the user's sequence \cite{xx}.
The training objective is formulated through an autoregressive model optimization problem:
\begin{equation}
\max_{\Phi} \sum_{(\bm{x},\bm{y})} \sum_{t=1}^{|y|} \log P_{\Phi}(y_t | \bm{x},\bm{y}_{\bm{<t}}),
\end{equation}
where $\Phi$ denotes the LLM's model parameters, $y_t$ represents the $t$-th token in the output sequence, and $y_{<t}$ includes all preceding tokens in the sequence. This objective ensures that each prediction is informed by both the prior items in the sequence and the detailed instructions describing the sequential recommendation task \cite{SeqRecSys, DL4SeqRec, LlaRA, CoLLM, E4SRec}.

% \textbf{Task Formulation.}
% The primary task of sequential recommendation is to predict the next item that aligns with user preference. For a user with a previous historical interaction sequence represented as $[i_1, i_2,...,i_n]$, the sequential recommender aims to forecast the subsequent item $i_{n+1}$ with which the user likely to interact.

% \textbf{Instruction Tuning.}
% To tune LLMs to comprehend and execute specific tasks guided by explicit instructions, instruction tuning changes the way LLMs are trained by structuring the training data into pairs of inputs and outputs, denoted as $(x, y)$. Here, $x$ represents a detailed textual instruction while $y$ is the expected output or response. 
% This method creates a coherent instructional framework that is essential for effective training. The LLMs are then fine-tuned on this data using an autoregressive training objective, which can be mathematically expressed as:
% \begin{equation}
% \max_{\Phi} \sum_{(x,y) \in \mathcal{Z}} \sum_{t=1}^{|y|} \log P_{\Phi}(y_t | x, y_{<t}),
% \end{equation}
% where \( \Phi \) denotes the parameters of the LLM, \( y_t \) represents the $t$-th token of the response, and \( y_{<t} \) denotes all preceding tokens.

% This autoregressive approach not only enhances the LLM's ability to follow detailed human directives, but fine-tunes its ability to interact in a human-like manner within specific instruction contexts as well, therefore improving the model's accuracy in producing relevant outputs.

% \textbf{Low-rank Adaptation (LoRA).}
\textbf{Fine-tuning with Low-rank Adaption (LoRA)}
Fully fine-tuning LLMs entails substantial computational resources \cite{Bert, GPT3, Llama, Llama2, mistral-7b, Alpaca, Vicuna}. LoRA emerges as an efficient alternative \cite{PEFT, PTuning, Prefixtuning, LoHA, LoKR, LoRA, IA3}, which injects trainable low-rank matrices into transformer layers to approximate the updates of pre-trained weights \cite{LoRA}. At its core, LoRA employs a low-rank decomposition where the update $\Delta \mathbf{W}$ to the pre-trained matrix $\mathbf{W_0} \in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}}$ is represented as $\Delta \mathbf{W} = \mathbf{BA}$.
% that modifies pre-trained matrices, such as those in attention mechanisms, for enhanced adaptability to specific tasks.
% Denoting the pre-trained matrix as \( \mathbf{W_0} \in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}} \), LoRA constrains its update amount after fine-tuning, denoted as $\Delta \mathbf{W}$, with a low-rank decomposition. That is, $\Delta \mathbf{W} = \mathbf{BA}$, 
% through the application of a low-rank decomposition. The formula for updating the matrix \( W \) can be succinctly expressed as:
% \begin{equation}
% W = W_0 + \Delta W = W_0 + BA,
% \end{equation}
% where $\mathbf{A} \in \mathbb{R}^{r \times d_{\text{in}}}$ and $\mathbf{B} \in \mathbb{R}^{d_{\text{out}} \times r}$ represent the low-rank components, and $r$, the LoRA rank, is significantly smaller than both $d_{\text{in}}$ and $d_{\text{out}}$, thereby ensuring the efficiency of the adaptation.
Here, $\mathbf{A} \in \mathbb{R}^{r \times d_{\text{in}}}$ and $\mathbf{B} \in \mathbb{R}^{d_{\text{out}} \times r}$ are the trainable low-rank matrices, and the rank of LoRA $r$ is significantly smaller than both $d_{\text{in}}$ and $d_{\text{out}}$, enhancing adaptation efficiency.

During the forward pass, the input $\Mat{x}$ is simultaneously multiplied by both $\mathbf{W_0}$ and $\Delta \mathbf{W}$, resulting in the output  $\mathbf{o}$:
\begin{equation}
\Mat{o} = \mathbf{W_0} \Mat{x} + \Delta \mathbf{W} \Mat{x} = \mathbf{W_0} \Mat{x} + \frac{\alpha}{r} \mathbf{BA} \Mat{x},
\end{equation}
where $\mathbf{W_0}$ remains frozen, and $\alpha$ is introduced as a scaling factor that adjusts the influence of the updates \wrt the original $\mathbf{W_0}$.

This methodology introduces a flexible and efficient means to customize these models to new tasks, circumventing the need for extensive retraining of all model parameters.

% \textbf{Hybrid Prompt for LLMs-based Sequential Recommendation.}
\textbf{Fine-tuning with Hybrid Prompting}
In the field of LLM-based sequential recommendation, a critical challenge is the divergence between the natural language space and the ``behavior'' space.
To bridge this gap, previous research \cite{LlaRA, E4SRec, CoLLM} introduces a hybrid prompt approach, which incorporates behavioral insights captured by recommendation models into the prompts.
This approach combines the textual token representation derived from the LLM's word embedding layer, with a behavior token representation learned from the recommender model with a cross-modal projector.
Formally, for an item $i$ with associated metadata $txt_i$, the LLM tokenizer and word embedding layer $\textbf{LLM-TKZ}(\cdot)$ convert it into token representations $\langle \textbf{emb}_t^{i} \rangle$:
\begin{equation}
    \langle \textbf{emb}_t^{i} \rangle = \textbf{LLM-TKZ}(txt_i).
\end{equation}
Concurrently, item $i$'s ID embedding $\Mat{e}_s^i$, pretrained using the encoder $\textbf{SR-EMB}(\cdot)$ of sequential recommender (\eg SASRec \cite{SASRec}, GRU4Rec \cite{GRU4Rec}), is represented as:
\begin{equation}
    \Mat{e}_s^i = \textbf{SR-EMB}(i;\theta_s).
\end{equation}
Then the ID embedding is transferred into a behavior token representation through a trainable projector $\textbf{Proj}(\cdot;\theta_p)$ to facilitate the alignment between the two modalities.
This alignment strategy enables LLMs to interpret and leverage the behavioral knowledge distilled by conventional recommenders \cite{LlaRA, CoLLM, E4SRec}.
Subsequently, the textual and behavioral token representations are then concatenated to form a comprehensive description of item $i$:
\begin{equation}
    \Mat{e}^{i} = \textbf{Concat}\left(\langle \textbf{emb}_t^{i} \rangle, \textbf{Proj}(\Mat{e}_s^i; \theta_p)\right).
\end{equation}

% by projecting the item embedding
% a projector to harmonize the collaborative signals with the linguistic structure of the language models. This integration of textual information with collaborative signals during training significantly augments the LLMs' ability to generate relevant recommendations.

% Central to this process is the transformation of the ID-based item representations, \( e_{s}^{i} \), through a trainable adapter. This adapter, a two-layer perceptron referred to as \( \textbf{Proj} \), reinterprets \( e_{s}^{i} \) within the linguistic framework of the LLM. The resulting behavioral token \( [\text{emb}_{s}^{i}] \) is denoted as:
% \begin{equation}
% [emb_s^{i}] = \textbf{Proj}(e_s^{i}; \theta_p),
% \end{equation}
% where \( \Theta_p \) represents the parameters of the trainable projector, to ensure precise alignment with the LLM's language space.

% Upon acquiring both the textual token \( [\text{emb}_{t}^{i}] \) and the behavioral token \( [\text{emb}_{s}^{i}] \) for a given item \( i \), the next step involves the integration of these two distinct yet complementary tokens. This integration is critical for constructing a richer, unified representation of each item. The concatenated representation is formulated as:
% \begin{equation}
% e_c^{i} = \textbf{Concat}([emb_t^{i}],[emb_s^{i}]),
% \end{equation}
% effectively merging the distinct characteristics captured by each token. This unified description not only enhances the item's representation within the LLM space but also improves LLM's accuracy in capturing user preferences and predicting future interactions.

% This manner effectively merge the distinct yet complementary characteristics captured by each token, thus enhancing the item representation within the LLM space and harness the potential of LLMs in the domain of sequential recommendation.


==> backup/3_methodology.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{figures/framework.png}
    \caption{The STARec framework. To implement sequence-customized activation patterns for various sequences, we integrate the strengths of MoE with LoRA. We utilize a trained sequence recommender \textbf{SR-EMB} to obtain representations, $seq-emb$, of the historical interaction sequences ($history ID-seq$). These representations serve as inputs to the \textbf{Gating Network}, which then determines customized activation weights, or contribution weights. These weights are used to perform a weighted summation of outputs from different experts to produce the final output $item_{n+1}$. In our prompts, we follow previous works by adopting a hybrid prompt approach that blends item-related collaborative information with textual data.}
    \label{fig:frameworkl}
\end{figure}

\wx{
\section{Methodology}

% In this section, we start with the formulation of LVLM instruction tuning and the analysis of the limitations of task experts. We then introduce the proposed MoCLE in detail. Figure 2 shows the overall framework of MoCLE.
% In this section, we provide a comprehensive description of our proposed framework. We begin with an overview in Section III-A. Subsequently, Section III-B delves into how MOELoRA seamlessly integrates the processes of MOE and LoRA, harnessing the strengths of both. The task-motivated gate function is detailed in Section III-C, where we also discuss the recovery of unique fine-tuned LLM parameters for each task. Lastly, Section III-D elaborates on the optimization and inference processes.

% To incorporate the behavioral patterns learned by traditional recommenders into LLMs, we propose a novel end-to-end framework, Large Language and Recommendation Assistant (LLaRA), as depicted in Figure 2. Specifically, beyond the text-only prompting, it exploits a hybrid prompting to align the behavioral representations, as derived from recommendation systems, with the language space of LLMs. It then employs curriculum learning — first focusing on text-only prompting, then gradually transitioning to hybrid prompting. This progressive strategy enables the LLM to familiarize the recommendation mechanism and internalize the behavioral knowledge of conventional recommenders. We now delve into the detailed architecture and training paradigm of LLaRA.
To address the issue of negative transfer associated with conventional LoRA fine-tuning, we introduce the Instance-wise LoRA (iLoRA) fine-tuning framework. This innovative approach adapts the Mixture of Experts (MoE) concept \cite{MOE1, MOE2} to tailor Large Language Models (LLMs) to individual characteristics in sequential recommendation, as illustrated in Figure \ref{fig:frameworkl}.
At the core is the integration of multiple experts, each encouraged to capture a specific aspect of user behaviors.
Different instances of user behavior (\ie item sequences) use a gating network to create instance-wise weights over experts.
Such weights instantiate the trainable matrices $\Mat{B}$ and $\Mat{A}$, thus personalizing a LoRA.
Upon this instance with its individually activated LoRA, We fine-tune the LLM to minimize the negative transfer among disparate sequences.
% Specifically, STARec extends the standard LoRA methods by subdividing the foundational LoRA module into a series of fine-grained experts. The core of STARec's functionality lies in its utilization of conventional sequential recommendation models to derive unique representations for each user sequence. These representations are subsequently channeled as inputs into an advanced gating network. By doing so, STARec effectively decomposes the complex recommendation task into distinct sub-tasks within a unified semantic space implicitly, tailored to the specifics of each sequence. This structured approach allows the LLMs to implement customized weight activation patterns that are optimally aligned with the various preferences and behaviors of users. In the following sections, we will delve into the detailed architecture and training paradigm of STARec, detailing how these elements synergistically contribute to its efficacy in delivering sequence-tailored recommendations.

% This method not only enriches the model’s understanding of user preferences but also significantly enhances its predictive accuracy. In the following sections, we will explore the delve into the detailed architecture and training paradigm of STARec, detailing how these elements synergistically contribute to its efficacy in delivering sequence-tailored recommendations.


\subsection{Instance-wise Generation for Sequential Recommendation}
Applying a uniform LoRA across the population of sequence instances risks overlooking individual variability and easily causes negative transfer, where distinct sequences might adversely affect each other.
This inspires us to view the modeling of each individual instance as a separate task instead, and customize instance-wise LoRA module.
By doing so, the LLM-based recommender is expected to align more closely with the behavioral and preference variability of individual users.
Formally, for any given instance $\bm{x}$, the autoregressive objective with instance-wise LoRA modules is as:
\begin{gather}
    \max_{\Delta\Phi} \sum_{(\bm{x},\bm{y})} \sum_{t=1}^{|y|} \log P_{\Delta\Phi(\bm{x})}(y_t | \bm{x},\bm{y}_{<t}),
\end{gather}
where $\Delta\Phi(\bm{x})$ yields $\bm{x}$-exclusive parameters, consisting of LLM's frozen weights and instance-wise LoRA's trainable weights.

To this end, one straightforward solution is to set up different LoRA modules for individual sequences, enabling each module to act as the expert tailored to its respective sequence.
However, it is impractical in terms of resource and time requirements, particularly as the number of sequences often reaches into the millions. This highlights the need for a more scalable solution to address the challenge of sequence-specific customization without excessive computational overhead.

\subsection{Instance-wise LoRA with the Mixture of Experts Concept}
Instead of establishing various LoRA modules, we implement the mixture-of-experts (MoE) concept \cite{MOE1,MOE2} to devise our instance-wise LoRA (iLoRA) framework.
This framework includes three components:
(1) Diverging from the standard LoRA module with up- and down-projection matrices, we divide each matrix into an array of experts, each encouraged to capture a distinct, hidden aspect of user behavior;
(2) For a given sequence instance, we use a gating network to obtain attention scores across the arrays of up- and down-projection experts, such that distinct sequences are likely to activate different experts;
(3) Such an attentive combination of up- and down-projection experts instantiates the weights of LoRA, which are individually customized for the instance of interest.
We will elaborate on these components one by one.


\subsubsection{Splitting Low-Rank Matrices into Experts}

Typically, the architectural foundation of LoRA is built upon two low-rank matrices: down-projection $\Mat{B} \in \mathbb{R}^{m \times r}$ and up-projection $\Mat{A} \in \mathbb{R}^{r \times d}$.
Here we meticulously divide each projection matrix into $N$ experts, as illustrated in Figure \ref{x}.
Each expert is intended to focus on capturing one specific, hidden aspect of user preference.
Formally, splitting the low-rank matrices is as follows:
\begin{gather}
    \Mat{B} = [\Mat{B}_1,\Mat{B}_2,\cdots,\Mat{B}_{K}],\quad\quad\Mat{A} = [\Mat{A}_1,\Mat{A}_2,\cdots,\Mat{A}_{K}],
\end{gather}
where $\Mat{B}_k\in\mathbb{R}^{d\times r^*}$ and $\Mat{A}_k\in\mathbb{R}^{r^*\times d}$ are the up- and down-projection pairs for the $k$-th expert, and $r^{*} = \frac{r}{K}$ is the partial rank determined by the total rank $r$ of LoRA and a predefined number of experts $K$.

By dividing individual LoRA modules into specialized experts, we ensure a more granular and precise adaptation to user preferences. This segmentation approach allows each expert to focus on specific aspects of user interaction patterns, thereby mitigating the risk of negative transfer that arises from generalized adaptations.
We should emphasize that such a segmentation scheme preserves the overall number of parameters equivalent to that of the standard LoRA, therefore preventing the potential overfitting issue.


\subsubsection{Generating Instance-wise Attentions over Experts}

Having obtained the experts (\ie up-projection submatrices $\{\Mat{B}_{k}\}_{k=1}^{K}$, down-projection submatrices $\{\Mat{A}_{k}\}_{k=1}^{K}$), we construct an instance-guided gating function to yield the contribution of each expert tailored to a specific sequence.
Specifically, for a sequence of historical items $\Mat{i}_{<n}=[i_1, i_2, \cdots, i_{n-1}]$, we utilize a sequential recommender (\eg SASRec \cite{SASRec}) to extract its representation as follows:
\begin{equation}
    \Mat{e} = \textbf{SR-EMB}(\Mat{i}_{<n};\theta_s).
\end{equation}
Here $\Mat{e}\in \mathbb{R}^{d}$ provides a holistic view of the user's behavioral patterns and preferences.
Subsequently, to ascertain the influence of each expert on distilling behavior patterns from this sequence, we get the contribution scores via a linear transformation with a softmax function:
\begin{equation}\label{eq:gating}
    \Mat{\omega} = \textbf{Softmax}(\Mat{W}_g \Mat{e}),
\end{equation}
where $\Mat{W}_g \in \mathbb{R}^{K \times d}$ is the trainable transformation matrix, and the softmax function ensures these contributions normalized as the attention scores, thereby preventing any single expert from disproportionately influencing the recommendation; $\Mat{\omega}$ represents the attention scores over all the experts, with the $k$-th element indicating the contribution of expert $K$.

By using the sequence representation as the guidance signal, we can get the instance-wise attentions over experts and encourage each expert's contribution closely aligned with the individual variability inherent in the sequence.
Moreover, distinct sequences tend to yield different attentions and activate different experts, while similar sequences incline towards analogous attentions.
This enforces the experts to specialize aspects of user behaviors.
By dynamically adapting to a wide range of user behaviors and preferences, these experts could specialize diverse aspects of user behaviors and be more adept at handling diverse user needs.


\subsubsection{Aggregating Mixture of Experts as Instance-wise LoRA}

For the instance $\Mat{i}_{<n}$ associated with the instance-wise attentions $\Mat{\omega}$, we use the mixture-of-experts concept to aggregate the up- and down-projection submatrices from different experts, so as to establish the instance-wise LoRA parameters:
\begin{gather}
    \Delta\Mat{W}(\Mat{i}_{<n})=\sum_{k=1}^{K}\omega_{k}\Mat{B}_{k}\Mat{A}_{k},
\end{gather}
where $\Delta\Mat{W}(\Mat{i}_{<n})$ encapsulates the adjustments enabled by our iLoRA. The attention score $\omega_{k}$, assigned by the gating network (\cf Equation \eqref{eq:gating}), reflects the relevance of expert $k$'s contribution to the particular sequence.

This dynamic adaptation of parameters ensures that our model remains flexible and responsive to the varied preferences and behaviors exhibited by users, effectively managing the complexity inherent in sequential recommendation systems. This approach not only enhances personalization but also improves the predictive accuracy of the recommendation system.


}

% % Sequential Recommendation as Multi-Task Generation
% \subsection{Sequential Recommendation as Multi-Task Generation}

% % 仿写MOELoRA 
% As previous mentioned in Figure \ref{fig:motivation}, merely applying a singular LoRA module to the sequential recommendation, risks oversimplifying the relationships between sequences, potentially leading to negative transfer effects where significantly different sequences adversely influence each other. In this work, we introduce STARec, a novel framework that re-conceptualizes sequential recommendation. We use the representation of sequences in the collaborative space to implicitly transform the recommendation task into a multi-task generation challenge.
% This approach mitigates the intrinsic complexities associated with the dynamic nature of user interactions and preferences. we consider a set of sequential recommendation tasks represented as $\mathbb{T} = [\mathcal{T}_1, \ldots, \mathcal{T}_i, \ldots, \mathcal{T}_M]$. The data corresponding to task $\Gamma_i$ is the unique sequence \( \mathcal{D}_i = s^{i} = [s_1, s_2, \ldots, s_m] \). Assuming the parameters of the LLM are represented by $\phi$, the multi-task fine-tuning challenge can be articulated as: Given the dataset of all sequences $\mathcal{D} = [\mathcal{D}_i]_{i=1}^{M}$, optimize the parameter $\phi$ of the LLM to ensure optimal performance across each sequence. The objective function for multi-task fine-tuning can be formulated as follows:
% \begin{equation}
% \max_{\Phi} \sum_{i \in [M]} \sum_{(x,y) \in \mathcal{D}_i} \sum_{t=1}^{|y|} \log P_{\Phi}(y_t | x, y_{<t}),
% \end{equation}


% \subsection{Customized Recommendation with STARec}

% After framing sequential recommendation as a multi-task generation challenge, we proceed to introduce the training and inference phases of STARec.

% \subsubsection{Finely Segmented LoRA}
% % 在这里提及通过细粒度的专家划分应对negative transfer
% % As 之前xx提及， 为了解决xx， 。。。
% As previously discussed, to tackle the challenge of negative transfer in sequence recommendation, we introduce a strategy of finely segmented LoRA modules. By dividing individual LoRA modules into specialized experts, we ensure a more granular and precise adaptation to user preferences. This segmentation approach allows each expert to focus on specific aspects of user interaction patterns, thereby mitigating the risk of negative transfer that arises from generalized adaptations.

% The architectural foundation of LoRA module is constructed from low-rank matrices $\Mat{B} \in \mathbb{R}^{m \times r}$ and $\Mat{A} \in \mathbb{R}^{r \times d}$. To enhance adaptability, we introduce a concept of finely segmented LoRA. Each matrix is meticulously divided into a set of experts weights. As we demonstrate in Figure 1, this structure is specifically designed to focus on learning the varied emphases within user preferences in the sequential dataset. In this manner, the subset block of LoRA module corresponding to the $i$-th expert is defined as:
% \begin{equation}
% \begin{split}
% \Mat{B_i} = \Mat{B}[:, (i-1)r^{*}:ir^{*}],
% \\
% \Mat{A_i} = \Mat{A}[:, (i-1)r^{*}:ir^{*}], 
% \end{split}
% \end{equation}
% where $\Mat{B_i}$ and $\Mat{A_i}$ denote the trainable blocks in matrices $\Mat{B}$ and $\Mat{A}$ for the $i$-th expert respectively. Here, the partial rank $r^{*}$ for each expert is determined by the total rank $r$ of LoRA and a predefined hyperparameter $n$, calculated as $r^{*} = \frac{r}{n}$.

% This finely segmented approach maintains the overall parameter count stable while enhancing the model's capacity to handle diverse and dynamic user behaviors. Each expert within the segmented LoRA modules is tailored to recognize and respond to distinct interaction features, enabling more accurate and effective personalization. This specialization ensures that the model not only preserves the integrity of the original parameter settings but also optimizes the responsiveness of each expert to the unique demands of different user sequences.

% \subsubsection{Sequence Guided Gate Function}

% In this section, we detail the intricacies of our sequence guided gate function. As previously emphasized, the contribution of each expert should be tailored to specific sequences. To manage the input from each expert appropriately, we implement a gating mechanism that uses item embeddings as guidance signals to allocate weights for each sequence. This mechanism is specifically designed to utilize the sequence representation, ensuring that the contribution weights are optimally tailored to the unique characteristics of each sequence. 

% We employ a sequential recommender, for example, SASRec, to extract latent representations from a sequence of interactions denoted by \( s^{i} = [s_1, s_2, \ldots, s_m] \). These interactions encompass a series of items. The process begins by transforming the interaction sequence \( s \) into a vector to acquire the hidden representation through:
% \begin{equation}
% e_{s}^{h} = \textbf{SR-EMB}(s^{i};\theta_e),
% \end{equation}
% where \( e_s^{h} \in \mathbb{R}^{d} \) represents the \( d \)-dimensional latent vector of the sequence \( s \). Here, \( d \) is typically set to values such as 64 or 256, depending on the model configuration. The \(\textbf{SR-EMB}(\cdot)\) is the encoding function of the sequential recommender, responsible for extracting a high-dimensional representation of the sequence \( s^{i} = [s_1, s_2, \ldots, s_m] \).
% % This vectorization facilitates the extraction of a deep, hidden representation of the sequence, which captures the underlying patterns and preferences implicit in the user's item interactions.By encoding user interaction sequences, we can obtain representations rich in collaborative information, which serve to effectively guide STARec in customizing parameter activation modes for distinct sequences. This process allows for tailored adjustments based on the nuanced patterns captured within the encoded data, enhancing the system's ability to deliver personalized recommendations by dynamically adapting its parameters to the specific characteristics of each sequence.

% Next, to quantify the influence of each expert on the final recommendation for a given sequence $s$, we compute the contribution weights through a linear transformation:
% \begin{equation}
% \omega_i = \textbf{Softmax}(\Mat{W_g} e_s^{h})
% \end{equation}
% where \( \omega_i \in \mathbb{R}^{n} \) denotes the vector of contribution weights for sequence \( s \), tailored specifically to leverage the diverse expertise within our model. The matrix \( \Mat{W_g} \in \mathbb{R}^{d \times n} \) serves as the transformation matrix. To ensure that no single expert disproportionately influences the recommendation, a softmax function is applied to normalize these weights, distributing influence equitably among the available experts.

% This strategy of employing sequence representation as guidance signals within the gate function not only aligns each expert's contribution with the sequence's unique characteristics but also enhances the overall effectiveness of the recommendation system. By dynamically adapting to a wide range of user behaviors and preferences, our model becomes more adept at handling diverse user needs.


% \subsubsection{Mixture of Experts}

% In our framework, the mixture of experts dynamically adjusts model parameter based on sequence information, aggregating contributions from different experts who capture the diverse preferences inherent in each sequence. This aggregation is weighted in a sequence-customized manner, ensuring each sequence's unique characteristics are optiomally represented.
% Compared to traditional MoE methods that directly feed the input vector $x$ into the gating network, our approach use the sequence representation as a guiding input for the gate function. For each unique sequence, this generates a sequence0tailored LoRA weight, specifically represented as:
% \begin{equation}
% \begin{split}
%     \Mat{W_s} &= \Mat{W_0} + \frac{\alpha}{r}\cdot \Delta \Mat{W} \\
%     &= \Mat{W_0} + \frac{\alpha}{r}\cdot \sum_{i=1}^{N}\omega_i \cdot E_i \\
%     &= \Mat{W_0} + \frac{\alpha}{r}\cdot \sum_{i=1}^{N}\omega_i \cdot \Mat{B_i}\Mat{A_i},
% \end{split}
% \end{equation}
% where \(\Mat{W_s}\) represents the sequence-specific parameters, \(\Mat{W_0}\) denotes the baseline parameters shared across all sequences, and \(\Delta \Mat{W}\) encapsulates the adjustments made by the STARec. Here, \(\omega_i\) represents the weights assigned by the gate function to each expert \(i\), reflecting the relevance of each expert's contribution to the specific sequence. \(E_i\) and \(\Mat{B_iA_i}\) signify the expert-specific transformation matrices, enhancing the model's ability to encode sequence-specific nuances.

% The dynamic adaptation of parameters ensures that our model remains flexible and responsive to the varied preferences and behaviors exhibited by users, effectively handling the complexity inherent in sequential recommendation systems.

==> backup/4_experiments.tex <==
\section{Experiments}

In this section, we first analyze the necessity of optimizing the current single LoRA module learning paradigm by transforming traditional sequential recommendation tasks into a multi-task learning framework. Following this theoretical groundwork, we proceed to empirically evaluate the efficacy of our proposed framework, \textbf{STARec}, across a spectrum of real-world datasets. In this evaluation, we meticulously compare STARec with a diverse array of baseline models, including conventional sequential recommender systems and LLM-based recommendation models. Moreover, we embark on a rigorous ablation study to dissect the underlying mechanisms propelling STARec's performance. Specifically, we delve into the intricate interplay between the sequence-representation-driven gate strategy embedded within STARec and its consequential impact on recommendation effectiveness.
To substantiate the merits of our framework in a rigorous academic manner, we meticulously formulate and address a series of research inquiries:
\begin{itemize}[leftmargin=*]
   \item \textbf{RQ1:} Does training a single LoRA module on sequential recommendation tasks induce negative transfer?
   
   \item \textbf{RQ2:} How does the performance of STARec compare with that of conventional sequential recommender models and LLM-based methods?

   \item \textbf{RQ3:} What impact the sequence guided gate function have on the fine-tuning process?
   
\end{itemize}

\textbf{Datasets.}
To validate the generalization ability of STARec, we conducted extensive experiments on four datasets derived from real-world recommendation scenarios: LastFM, GoodReads, Amazon-book, and Steam (the statistics of datasets are illustrated in Appendix A) :

\begin{itemize}[leftmargin=*]
\item \textbf{LastFM}
% from LlaRA
Collected from the Last.fm online music platform, includes user-artist listening relationships and the names of artists.
\item \textbf{MovieLens}
% from LlaRA
A commonly-used movie recommendation dataset that contains user ratings and movie titles.
\item \textbf{Amazon-book}
Contains user reviews and interactions with books available on the Amazon platform.
\item \textbf{Steam}
% from LlaRA
Encompasses user reviews for video games on the Steam Store, in addition to game titles.

\end{itemize}

\textbf{Baselines.} 
% 需修改
We compared STARec with several models, including traditional sequential recommendation models and those based on Large Language Models (LLMs), such as GRU4Rec\cite{GRU4Rec}, Caser, SASRec\cite{SASRec}, Llama2\cite{Llama2}, GPT-4, MoRec, TallRec\cite{TallRec}, and LlaRA\cite{LlaRA}. GRU4Rec, Caser, and SASRec utilize recurrent neural networks, convolutional neural networks, and Transformer encoders, respectively, to capture sequential patterns in user behavior. Llama2, a well-known open-source LLM, is released by Meta, and in our experiments, we utilized the 7B version. GPT-4, the latest version of the GPT series, is a milestone in the performance of LLMs across diverse tasks, from natural language processing to other domains. We conducted our research using the API provided by OpenAI. MoRec enhances traditional sequential recommendation models, such as text-based features, by leveraging pretrained modal encoders to strengthen the modal characteristics of encoded items. TallRec guides LLMs through fine-tuning on recommendation corpora. LlaRA further improves the recommendation effectiveness of LLMs by aligning collaborative signals to the text space through a hybrid prompt method.

\begin{table*}[t]
\caption{The Results of STARec compared with traditional sequential recommender models and LLMs-based methods.}
\vspace{-5pt}
\label{tab:overall}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
\multicolumn{1}{c|}{} & \multicolumn{3}{c|}{LastFM} & \multicolumn{3}{c|}{MovieLens} & \multicolumn{3}{c|}{Amazon-book} & \multicolumn{3}{c}{Steam} \\
\midrule
\multicolumn{1}{c|}{} & ValidRatio & HitRatio@1 & Imp.\% & ValidRatio & HitRatio@1 & Imp.\% & ValidRatio & HitRatio@1 & Imp.\% & ValidRatio & HitRatio@1 & Imp.\% \\
\midrule
\multicolumn{13}{c}{\textbf{Traditional}} \\
\midrule
GRU4Rec   & 1.0000 & 0.2616 & 84.86\% & 1.0000 & 0.3750 & 36.21\% & 1.0000 & - & -\% & 1.0000 & 0.4168 & -\% \\
Caser     & 1.0000 & 0.2233 & 116.57\% & 1.0000 & 0.3861 & 32.30\% & 1.0000 & - & -\% & 1.0000 & 0.4368 & -\% \\
SASRec    & 1.0000 & 0.2233 & 116.57\% & 1.0000 & 0.3444 & 48.32\% & 1.0000 & - & -\% & 1.0000 & 0.4010 & -\% \\
\midrule
\multicolumn{13}{c}{\textbf{LLM-based}} \\
\midrule
Llama2    & 0.3443 & 0.0246 & 1865.85\% & 0.4421 & 0.0421 & 1113.30\% & - & - & -\% & 0.1653 & 0.0135 & -\% \\
ChatRec     & 1.0000 & 0.3770 & 28.28\% & 0.9895 & 0.2000 & 155.40\% & - & - & -\% & 0.9798 & 0.3626 & -\% \\
MoRec     & 1.0000 & 0.1652 & 192.74\% & 1.0000 & 0.2822& 81.01\% & - & - & -\% & 1.0000 & 0.3911 & -\% \\
TALLRec   & 0.9836 & 0.4180 & 15.69\% & 0.9263 & 0.3895 & 31.14\% & - &  -& -\% & 0.9840 & 0.4637 & -\% \\
LLaRA(SASRec) & 1.0000 & 0.4508 & 7.28\% & 0.9684 & 0.4421 & 15.53\% & 0.9927 & 0.3668 & 5.75\% & 0.9975 & 0.4949 & -\% \\
\midrule
\multicolumn{13}{c}{\textbf{Ours}} \\
\midrule
STARec(SASRec) & 1.0000 & \textbf{0.5000} & - & 0.9891 & \textbf{0.5275} & - & - & \textbf{0.3879}
 & - & - & - & - \\
\bottomrule
\end{tabular}}
\vspace{-15pt}
\end{table*}

\textbf{Training Protocol.}
% from LlaRA
For our study, we opt for Llama2-7B \cite{Llama2} as the LLM backbone. Given the disparity in computational resources between traditional sequential recommendation models and LLM-based methods, we execute baseline models on a single Nvidia A40, while LLaRA is implemented on a single Nvidia-smi A100. This ensures optimal utilization of available computational resources. All implementations are carried out using Python 3.8 and PytorchLightning 1.8.6.


\textbf{Evaluation Protocol.}
To evaluate STARec and baseline models, we construct candidate sets for each sequence by randomly selecting 20 non-interacted items and ensuring the inclusion of the correct next item. The models aim to identify this correct item from the candidate set, and their performance is measured using the HitRatio@1 metric. LLM-based recommenders, given proper prompts, generate a single candidate item, while traditional models are adapted to this setting by selecting the item with the highest probability. Since generative approach can produce invalid responses, such as nonsensical words or items outside the candidate sets, we introduce an additional metric, Valid Ratio, which quantifies the proportion of valid responses (i.e., items in the candidate set) across all sequences. This metric evaluates the models’ ability to follow instructions accurately.

To assess the performance of STARec and baseline models, we construct candidate sets for each sequence by randomly selecting 20 non-interacted items while ensuring the inclusion of the correct next item. Performance is evaluated using the HitRatio@1 metric, wherein models attempt to identify the correct item from the candidate set. LLM-based recommenders, when provided with appropriate prompts, generate a single candidate item. Conversely, traditional models are adapted to select the item with the highest probability. Additionally, we introduce the Valid Ratio metric to quantify the proportion of valid responses (i.e., items within the candidate set) across all sequences. This metric serves to evaluate the models' adherence to instructions accurately.

\subsection{Investing Multi-Task Optimization in Sequential Recommendation (RQ1)}

Existing research on LLM-based recommendation systems often simplifies the approach by using a single LoRA module to train on all recommendation data, overlooking the issue of gradient conflict (defined as negative cosine similarity between gradients) and its resulting negative transfer. We conduct experiments on LoRA to investigate how gradients interact within diverse sequence environments.

\subsubsection{Experiment Setup}

We extend the previous research setup to train models on multi-task scenarios\cite{xx}. Specifically, we jointly train recommendation sequences in a basic LoRA training framework. We use an effective batch sizes of 128 sequences. The recommendation sequences are divided into multiple tasks using representations derived from the sequential recommendation model SASRec, with a dimension of 64.

To investigate large-scale multi-tasking in sequential recommendation tasks, we sample 40k sequences from the Steam dataset. We clustered these sequences into 8 sub-datasets using Euclidean distance. At checkpoints across 1k training steps, we measured the pairwise cosine similarity of model gradients for all sequences. We averaged the LoRA gradients that were bound to the same modules, such as $gate proj$.

\subsubsection{Observation}
% 仿写
Gradient similarity reflects the proximity of recommendation sequences. We explored whether similar sequential recommendation tasks exhibit similar loss geometries and vice versa. To achieve this, we used Euclidean distance to control task similarity and gradient similarity to measure loss geometry. In Figure \ref{fig:motivation}, a symmetric heatmap visually displays the average gradient similarity across all checkpoints at different training steps. Specifically, we observed strong clustering along the diagonal of the gradient similarity matrix for sets of recommendation sequences that are closely related in the Euclidean space. Conversely, recommendation sequences that are distant in Euclidean space exhibit correspondingly lower gradient similarity, leading to negative transfer.

This implies that sequential recommendation tasks with large Euclidean distances from each other will negate each other, resulting in poorer updates for a subset of, or even for all sequences. Similarly, imbalanced loss scales may cause sequences with smaller losses to be dominated by those with larger losses.

\subsubsection{Case Study}

\subsection{Performance Comparison (RQ2)}

This section entails a comprehensive comparison of STARec against both traditional and LLM-based baselines. We conduct a holistic evaluation, considering metrics of both HitRatio@1 and Valid Ratio across LastFM, MovieLens, Amazon-book, and Steam datasets to demonstrate the effectiveness and robustness of STARec.

We have integrated the STARec framework with item embeddings obtained from SASRec. Comparative analysis of STARec against these baseline models, as detailed in Table \ref{tab:overall}, reveals that STARec consistently outperforms all the baseline models across four datasets. Specifically, STARec achieves the highest HitRatio@1 metrics of 0.4836, 0.5108, and 0.3879 on the LastFM, MovieLens, and Amazon-book datasets, respectively, with comparable superior performance on the MovieLens dataset. These results underscore the efficacy of leveraging sequence representations as guidance signals to fine-tune LoRA parameters, thereby enabling personalized recommendations at the parameter level.

\subsection{Ablation Study (RQ3)}

Our research has demonstrated the effectiveness of using sequence embeddings as guidance signals in LLM-based recommendation systems to customize different activation patterns for various sequences. Subsequently, this section discusses the impact of sequence representation as a guidance signal in the MOE approach. We conducted experiments employing two strategies:
\begin{itemize}[leftmargin=*]
    \item \textbf{Random Embedding:}
    Employing random embeddings throughout both training and inference to activate expert weights.
    \item \textbf{STARec (sequence-tailored guidance signal):}
    Utilizing sequence representation proposed by the STARec framework as the guidance signal.
   
\end{itemize}
% from LLaRA
The comparative experimental results of the two strategies are presented in Table \ref{}. A careful analysis of the results reveals that our proposed method, STARec, consistently outperforms the other baseline methods across both datasets. This demonstrates the rationale for using user representation as a guidance signal, as the MOE expert modules indeed received sequence-specific guidance based on the user representation.
% 消融
% random-embedding vs SAS-embedding

==> chapters/5_related_work.tex <==
\section{Related Work}

\textbf{Large Language Models}
Recent years have witnessed a surge of activity in language modeling research, establishing it as a cornerstone for both understanding and generating language. This momentum has given rise to a new breed of language models (LMs), including notable works such as BERT \cite{Bert}, GPT-3 \cite{GPT3}, LLama \cite{Llama}, LLama2 \cite{Llama2}, Mistral-7B \cite{mistral-7b}, Alpaca \cite{Alpaca}, and Vicuna \cite{Vicuna}. These LMs, predominantly based on the Transformer architecture, have demonstrated remarkable versatility, exemplified by models like BERT \cite{Bert} and T5 \cite{T5}, owing to their extensive training corpus.
A significant stride in this domain has been the exploration of scaling effects, with researchers pushing the boundaries by augmenting both the parameter and training corpus scales to unprecedented magnitudes, encompassing billions of parameters and trillions of training tokens \cite{Llama, Llama2, Vicuna, GPT3, judging}. These Large Language Models (LLMs) exhibit substantial performance enhancements and showcase unique capabilities, including but not limited to common sense reasoning and instruction following.
Moreover, the development of domain-specific LLMs further enriches this landscape. Models tailored to specific domains, such as finance \cite{BloombergGPT}, medicine \cite{clinic}, biochemistry \cite{c6LLM4Molecular} and law \cite{law}, amalgamate domain expertise with the inherent commonsense knowledge of general LLMs. These advancements not only broaden the scope of LLM applications but also inspire exploration into their potential utility in recommendation systems.

\textbf{Mixture of Experts}
Mixture of Experts. MoE models \cite{MOE0, MOE1, MOE2} are considered as an effective way to increasing the model capacity in terms of parameter size. In MoE, certain parts of the model are activated while the computation is kept the same or close to its dense counterpart. Recently, it has been thoroughly investigated in the field of computer vision \cite{MOEvision1, MOEvision2}, natural language processing \cite{MOEnlp1, MOEnlp2} and multi-modal learning \cite{MOEmulti1, MOEmulti2}.


\section{Broader Impact}

==> chapters/8_checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The claims made in the abstract and introduction accurately reflect the contributions and scope of our paper. The abstract succinctly summarizes our approach, the Instance-wise Low-Rank Adaptation (iLoRA), and its application in sequential recommendation systems. It also highlights the integration with the Mixture of Experts (MoE) framework, providing a clear overview of the method's novelty and effectiveness. The introduction elaborates on the motivation, background, and significance of our contributions, ensuring that the claims align with the detailed discussions and results presented in the subsequent sections of the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the limitations of the work performed in limitation \ref{limitation}. By explicitly acknowledging these limitations, we provide a balanced view of our work and suggest directions for future research to address these challenges.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: we provide the full set of assumptions and a complete (and correct) proof in our methodology part \ref{method}. The assumptions are clearly stated, and the proofs are detailed to ensure correctness and reproducibility. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We fully disclose all the information needed in Appendix \ref{sec:app-settings} and Appendix \ref{appendix:mot_setup}. This includes details about the datasets, experimental setups, hyperparameters, and evaluation metrics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide open access to the data and code. And we explain our set in Appendix \ref{sec:app-settings} and Appendix \ref{appendix:mot_setup}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We specify all the training and test details in Appendix \ref{appendix:mot_setup} and Appendix \ref{sec:app-settings}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do it in the Appendix \ref{sta}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: For each experiment we proviede sufficient information in our experiments part, Appendix \ref{sta}, Appendix \ref{appendix:mot_setup}, Appendix \ref{sec:app-settings}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our research fully conforms to the NeurIPS Code of Ethics. We have carefully reviewed the guidelines and ensured that all aspects of our research, from data collection and usage to experimental conduct and reporting, adhere to ethical standards. We maintain transparency in our methodology, respect for privacy, and fairness in our experimental design, ensuring that our work aligns with the ethical principles outlined by NeurIPS.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper discusses the potential positive and negative societal impacts of our work in the "Broader Impacts" section. By acknowledging these impacts, we provide a balanced view of our work and suggest mitigation strategies to address potential negative outcomes.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We conduct experiments on recommendation tasks using publicly available datasets and build upon existing open-source methods. Therefore, the risk of misuse is minimal, and specific safeguards for data or model release are not necessary. Our focus remains on transparency and reproducibility, ensuring that our work can be used responsibly by the research community.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We fully adhere to these requirements by properly crediting the creators or original owners of all assets used in our paper. Each asset, including datasets, code, and models, is accompanied by a citation to the original source, and the specific versions used are stated. We explicitly mention the licenses and terms of use for each asset, ensuring compliance with their respective usage guidelines.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We offer our code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:We are not involved in these risks as we are only engaged in recommendation tasks. Our research does not include crowdsourcing experiments or research with human subjects, thus this question is not applicable to our paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We are not involved in these risks as we are only engaged in recommendation tasks. Our research does not involve human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}
